Multi-fidelity surrogate modeling for time-series outputs

This paper considers the surrogate modeling of a complex numerical code in a multifidelity framework when the code output is a time series. Using an experimental design of the low-and high-fidelity code levels, an original Gaussian process regression method is proposed. The code output is expanded on a basis built from the experimental design. The first coefficients of the expansion of the code output are processed by a co-kriging approach. The last coefficients are collectively processed by a kriging approach with covariance tensorization. The resulting surrogate model taking into account the uncertainty in the basis construction is shown to have better performance in terms of prediction errors and uncertainty quantification than standard dimension reduction techniques.

==> Abstract__1_.tex <==
This paper considers the surrogate modeling of a complex numerical code in a multi-fidelity framework when the code output is a time series \textcolor{black}{and two code levels are available: a high-fidelity and expensive code level and a low-fidelity and cheap code level.}
\textcolor{black}{The goal is to emulate a fast-running approximation of the high-fidelity code level.}
\textcolor{black}{A}n original Gaussian process regression method is proposed \textcolor{black}{that uses} an experimental design of the low- and high-fidelity code levels.
The code output is expanded on a basis built from the experimental design.
The first coefficients of the expansion of the code output are processed by a co-kriging approach.
The last coefficients are processed by a kriging approach with covariance tensorization.
The resulting surrogate model \textcolor{black}{provides a predictive mean and a predictive variance of the output of the high-fidelity code level.}
\textcolor{black}{It} is shown to have better performance in terms of prediction errors and uncertainty quantification than standard dimension reduction techniques.

==> Statement.tex <==


In this work, we introduce an original approach to the construction of a surrogate model in the framework of hierarchical multi-fidelity codes with time-series outputs.
The main idea is to combine a reduction method of the output dimension, that fits well with the autoregressive model of multi-fidelity co-kriging, and a simple fidelity method that allows to treat time series output by Gaussian process regression  with covariance tensorization.
In \Cref{sec::Regressiontools} we give the main elements of the Gaussian process regression theory that are needed in our paper.

The choice of the basis for dimension reduction is crucial.
In Sections \ref{sec::AR1multiproj}-\ref{sec::AR1multiTens} we develop an empirical method based on K-fold cross-validation which uses only low-fidelity data and allows us to consider the first two moments of the basis vectors. 
Once projected onto the reduced space it is possible to characterise the models of the first coefficients of the expansion of the code output onto the basis by the multi-fidelity Gaussian process regression method.

The orthogonal part, which is the projection of the code output onto the orthogonal space of the reduced space, can be neglected if the dimension of the reduced space can be chosen so as to achieve a good bias-variance trade-off (see \Cref{sec::AR1multiproj}) or it can be treated by Gaussian process regression with covariance  tensorization (see \Cref{sec::AR1multiTens}).
The latter approach collectively addresses the orthogonal part of the high-fidelity code and it makes it possible  to better predict the output of the high-fidelity code and to better quantify the uncertainty of the prediction.

The results presented in the numerical example in \Cref{sec::Illustration} confirm that the processing of the orthogonal part is important.
In this example we test the different methods presented in the paper and we assess their performance in terms of prediction errors and uncertainty quantification.
